Constellations in prime elements of number fields

Given any number field, we prove that there exist arbitrarily shaped constellations consisting of pairwise non-associate prime elements of the ring of integers. This result extends the celebrated Green-Tao theorem on arithmetic progressions of rational primes and Tao's theorem on constellations of Gaussian primes. Furthermore, we prove a constellation theorem on prime representations of binary quadratic forms with integer coefficients. More precisely, for a non-degenerate primitive binary quadratic form $F$ which is not negative definite, there exist arbitrarily shaped constellations consisting of pairs of integers $(x,y)$ for which $F(x,y)$ is a rational prime. The latter theorem is obtained by extending the framework from the ring of integers to the pair of an order and its invertible fractional ideal.

==> root_2_points_new2.tex <==
\filldraw[lightgray!50] (\lowerr,\lowerr)--({ln(1000 )/2},{ln(1000 )/2})
-- ++({ln(1+sqrt(2))},{ln(sqrt(2)-1)})--({\lowerr+2*(ln(1+sqrt(2)))},\lowerr );
\draw[thin] ( {ln(1000 )- \upperr}, \upperr )
 --( \upperr , {ln(1000 )- \upperr} );
\node[fill=black,shape=circle,inner sep=0.1pt] at(0.346574,0.346574){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(0.881374,-0.881374){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.039721,1.039721){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.342454,0.603456){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.574521,-0.188226){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.445186,1.445186){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.656825,1.176388){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.831403,0.807654){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.979986,0.217239){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.732868,1.732868){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.895647,1.538340){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.035601,1.296603){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.158351,0.977143){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.267668,0.504921){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.956012,1.956012){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.088286,1.803535){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.205090,1.623551){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.309667,1.403905){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.404335,1.122025){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.490811,0.728064){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.138333,2.138333){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.249741,2.012939){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.349972,1.869535){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.441066,1.702068){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.524550,1.500801){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.601599,1.248549){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.673133,0.910386){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.292484,2.292484){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.388716,2.185995){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.476496,2.066799){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.557188,1.931448){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.631853,1.774867){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.701327,1.589132){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.766287,1.360847){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.827284,1.064537){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.426015,2.426015){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.510713,2.333474){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.588794,2.231487){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.661218,2.117906){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.728748,1.989750){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.792006,1.842723){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.851499,1.670290){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.907650,1.461798){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.960815,1.198068){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.543798,2.543798){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.619432,2.461972){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.689745,2.372850){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.755438,2.275000){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.817079,2.166527){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.875141,2.044840){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.930016,1.906266){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.982035,1.745353){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.031482,1.553486){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.078598,1.315851){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.649159,2.649159){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.717481,2.575824){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.781433,2.496682){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.841540,2.410734){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.898237,2.316699){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.951892,2.212894){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.002814,2.097053){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.051268,1.966012){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.097482,1.815173){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.141655,1.637468){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.183959,1.421212){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.744469,2.744469){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.806770,2.678027){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.865416,2.606855){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.920812,2.530226){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.973300,2.447235){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.023170,2.356727){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.070670,2.257206){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.116017,2.146674){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.159395,2.022388){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.200970,1.880434){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.240886,1.714941){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.279269,1.516522){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.831480,2.831480){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.888735,2.770747){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.942888,2.706086){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.994259,2.636952){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.043120,2.562682){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.089704,2.482451){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.134214,2.395216){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.176827,2.299637){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.217698,2.193948){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.256964,2.075755){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.294746,1.941696){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.331153,1.786841){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.366280,1.603533){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.911523,2.911523){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.964488,2.855595){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.014788,2.796353){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.062679,2.733378){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.108381,2.666170){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.152085,2.594118){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.193959,2.516468){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.234150,2.432277){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.272787,2.340341){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.309987,2.239089){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.345853,2.126418){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.380477,1.999421){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.413942,1.853916){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.446323,1.683576){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.985631,2.985631){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.034904,2.933803){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.081864,2.879142){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.126716,2.821319){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.169643,2.759946){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.210803,2.694559){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.250335,2.624595){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.288364,2.549366){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.325000,2.468014){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.360340,2.379453){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.394474,2.282279){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.427482,2.174637){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.459435,2.053994){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.490398,1.916774){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.520431,1.757684){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.054624,3.054624){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.100687,3.006336){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.144721,2.955598){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.186898,2.902147){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.227368,2.845677){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.266263,2.785826){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.303702,2.722164){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.339790,2.654171){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.374621,2.581217){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.408279,2.502518){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.440841,2.417092){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.472376,2.323681){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.502947,2.220638){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.532612,2.105743){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.561421,1.975913){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.589424,1.826677){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.119162,3.119162){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.162408,3.073962){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.203860,3.026621){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.243663,2.976927){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.281941,2.924635){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.318809,2.869455){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.354365,2.811053){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.388700,2.749027){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.421896,2.682898){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.454024,2.612084){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.485153,2.535870){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.515342,2.453366){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.544646,2.363437){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.573115,2.264615){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.600797,2.154945){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.627733,2.031749){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.653962,1.891215){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.179787,3.179787){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.220540,3.137303){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.259696,3.092933){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.297378,3.046503){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.333690,2.997812){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.368730,2.946628){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.402584,2.892682){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.435329,2.835659){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.467036,2.775187){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.497768,2.710822){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.527584,2.642027){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.556537,2.568147){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.584675,2.488370){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.612042,2.401673){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.638681,2.306740){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.664629,2.201840){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.689920,2.084632){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.714587,1.951840){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.236945,3.236945){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.275477,3.196869){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.312579,3.155120){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.348354,3.111551){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.382892,3.065997){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.416278,3.018269){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.448585,2.968147){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.479881,2.915381){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.510226,2.859674){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.539679,2.800681){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.568288,2.737987){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.596102,2.671099){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.623163,2.599414){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.649511,2.522190){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.675182,2.438500){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.700211,2.347161){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.724629,2.246633){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.748465,2.134858){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.771745,2.008998){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.291013,3.291013){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.327553,3.253086){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.362805,3.213665){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.396857,3.172625){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.429787,3.129829){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.461667,3.085118){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.492562,3.038315){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.522531,2.989214){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.551629,2.937576){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.579903,2.883127){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.607400,2.825540){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.634161,2.764434){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.660224,2.699350){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.685626,2.629732){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.710398,2.554904){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.734571,2.474019){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.758174,2.386012){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.781232,2.289506){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.803771,2.182681){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.825813,2.063065){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.342306,3.342306){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.377051,3.306310){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.410628,3.268971){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.443115,3.230183){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.474580,3.189829){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.505085,3.147778){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.534687,3.103881){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.563437,3.057968){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.591384,3.009846){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.618572,2.959290){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.645039,2.906041){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.670824,2.849797){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.695961,2.790200){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.720482,2.726824){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.744415,2.659159){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.767789,2.586581){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.790630,2.508320){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.812960,2.423410){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.834802,2.330616){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.856178,2.228322){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.877106,2.114359){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.391096,3.391096){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.424213,3.356844){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.456269,3.321378){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.487329,3.284607){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.517453,3.246432){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.546696,3.206742){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.575108,3.165411){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.602735,3.122298){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.629620,3.077242){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.655800,3.030060){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.681313,2.980542){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.706191,2.928442){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.730465,2.873479){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.754163,2.815318){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.777313,2.753564){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.799940,2.687744){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.822065,2.617285){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.843712,2.541483){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.864900,2.459459){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.885648,2.370102){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.905974,2.271970){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.925896,2.163149){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.437616,3.437616){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.469252,3.404947){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.499917,3.371174){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.529670,3.336221){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.558563,3.300002){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.586645,3.262422){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.613959,3.223374){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.640548,3.182739){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.666447,3.140382){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.691693,3.096152){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.716317,3.049875){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.740349,3.001351){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.763818,2.950353){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.786748,2.896613){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.809164,2.839821){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.831088,2.779608){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.852543,2.715535){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.873546,2.647075){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.894118,2.573581){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.914274,2.494254){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.934033,2.408088){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.953409,2.313792){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.972416,2.209669){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.701966,3.199771){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.726342,3.158145){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.750137,3.114711){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.773379,3.069304){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.796094,3.021737){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.818304,2.971794){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.840031,2.919224){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.861296,2.863738){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.882119,2.804990){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.902516,2.742575){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.922506,2.676003){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.942104,2.604681){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.961326,2.527879){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.980185,2.444684){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.998694,2.353935){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.016868,2.254121){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.848894,3.041715){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.869974,2.992784){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.890618,2.941336){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.910845,2.887096){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.930671,2.829744){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.950111,2.768902){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.969180,2.704118){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.987893,2.634843){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.006262,2.560410){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.024300,2.479988){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.042018,2.392529){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.059427,2.296680){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.938769,2.962968){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.958054,2.909920){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.976974,2.853900){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.995543,2.794554){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.013773,2.731463){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.031677,2.664122){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.049266,2.591916){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.066551,2.514088){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.083542,2.429688){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.100249,2.337502){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.021228,2.877486){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.039000,2.819565){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.056462,2.758081){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.073624,2.692568){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.090496,2.622460){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.107089,2.547064){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.123411,2.465516){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.139470,2.376723){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.097403,2.784009){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.113882,2.720227){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.130094,2.652098){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.146047,2.578986){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.161750,2.500104){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.177210,2.414463){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.152582,2.747141){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.168183,2.680883){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.183545,2.609921){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.198674,2.533536){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.213578,2.450831){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.219687,2.639928){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.234283,2.565887){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.248669,2.485922){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.268668,2.597223){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.282571,2.519824){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.315361,2.552614){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(0.000000,0.000000){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(0.693147,0.693147){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.227947,-0.534800){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.098612,1.098612){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.484830,0.461080){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.386294,1.386294){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.689028,0.950030){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.921094,0.158347){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.609438,1.609438){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.858516,1.276978){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.057762,0.775452){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.791759,1.791759){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.003399,1.522962){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.177977,1.154228){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.326559,0.563812){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(1.945910,1.945910){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.129922,1.720225){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.285279,1.428293){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.419714,1.014273){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.079442,2.079442){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.242221,1.884914){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.382175,1.643177){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.504925,1.323716){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.614242,0.851494){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.197225,2.197225){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.343172,2.026276){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.470506,1.819954){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.583442,1.559693){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.684908,1.206912){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.302585,2.302585){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.434859,2.150108){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.551664,1.970125){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.656240,1.750479){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.750909,1.468599){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.837385,1.074638){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.397895,2.397895){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.518842,2.260281){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.626726,2.100661){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.724097,1.910632){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.812822,1.675815){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.894312,1.368368){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.484907,2.484907){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.596315,2.359512){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.696546,2.216109){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.787640,2.048642){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.871124,1.847375){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.948172,1.595122){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.019707,1.256959){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.564949,2.564949){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.668215,2.449779){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.761808,2.319597){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.847385,2.169894){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.926214,1.993767){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.999279,1.779844){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.067368,1.507343){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.639057,2.639057){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.735290,2.532568){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.823070,2.413372){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.903762,2.278022){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.978426,2.121440){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.047901,1.935706){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.112861,1.707421){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.173857,1.411110){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.708050,2.708050){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.798148,2.609024){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.880794,2.499103){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.957129,2.375590){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.028047,2.234643){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.094268,2.070518){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.156374,1.874064){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.214848,1.629340){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.772589,2.772589){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.857287,2.680048){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.935368,2.578061){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.007791,2.464479){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.075322,2.336324){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.138579,2.189297){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.198072,2.016864){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.254223,1.808372){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.307389,1.544642){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.833213,2.833213){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.913123,2.746359){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.987117,2.651238){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.056011,2.546108){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.120462,2.428614){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.181011,2.295453){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.238101,2.141796){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.292108,1.960166){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.343346,1.738058){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.890372,2.890372){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.966005,2.808546){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.036319,2.719423){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.102011,2.621574){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.163653,2.513101){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.221715,2.391414){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.276589,2.252840){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.328609,2.091926){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.378055,1.900059){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.425172,1.662425){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.944439,2.944439){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.016231,2.867091){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.083213,2.783255){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.145989,2.691742){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.205055,2.591003){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.260826,2.478967){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.313651,2.352776){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.363824,2.208330){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.411600,2.039438){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.457197,1.836108){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(2.995732,2.995732){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.064055,2.922397){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.128007,2.843255){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.188113,2.757308){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.244811,2.663272){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.298466,2.559468){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.349388,2.443626){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.397842,2.312585){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.444056,2.161746){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.488229,1.984042){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.530532,1.767785){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.044522,3.044522){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.109695,2.974804){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.170879,2.899858){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.228535,2.818838){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.283046,2.730669){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.334739,2.633968){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.383891,2.526905){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.430740,2.406991){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.475492,2.270712){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.518326,2.112886){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.559401,1.925396){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.091042,3.091042){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.153343,3.024601){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.211989,2.953429){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.267386,2.876800){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.319874,2.793809){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.369743,2.703301){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.417244,2.603779){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.462590,2.493247){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.505969,2.368962){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.547544,2.227008){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.587459,2.061515){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.625842,1.863095){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.135494,3.135494){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.195165,3.072035){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.251476,3.004274){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.304783,2.931586){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.355393,2.853197){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.403564,2.768137){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.449520,2.675163){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.493457,2.572651){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.535545,2.458416){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.575933,2.329429){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.614752,2.181306){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.652121,2.007361){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.178054,3.178054){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.235309,3.117321){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.289462,3.052659){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.340833,2.983526){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.389693,2.909256){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.436277,2.829024){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.480787,2.741789){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.523400,2.646211){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.564271,2.540522){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.603537,2.422329){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.641320,2.288270){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.677726,2.133415){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.712854,1.950107){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.218876,3.218876){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.273902,3.160644){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.326058,3.098811){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.375628,3.032901){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.422856,2.962338){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.467954,2.886416){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.511106,2.804252){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.552472,2.714728){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.592195,2.616395){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.630400,2.507327){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.667200,2.384890){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.702692,2.245343){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.736968,2.083114){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.258097,3.258097){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.311062,3.202168){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.361362,3.142926){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.409253,3.079952){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.454955,3.012744){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.498659,2.940692){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.540533,2.863042){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.580723,2.778851){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.619361,2.686915){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.656561,2.585662){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.692427,2.472991){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.727050,2.345994){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.760515,2.200490){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.792897,2.030149){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.295837,3.295837){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.346889,3.242037){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.395462,3.185177){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.441784,3.124889){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.486055,3.060731){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.528449,2.992173){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.569118,2.918566){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.608198,2.839108){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.645808,2.752787){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.682054,2.658305){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.717033,2.553956){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.750829,2.437435){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.783520,2.305524){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.815177,2.153531){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.332205,3.332205){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.381478,3.280377){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.428437,3.225715){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.473290,3.167892){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.516217,3.106520){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.557377,3.041133){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.596909,2.971169){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.634938,2.895940){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.671573,2.814588){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.706914,2.726026){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.741048,2.628853){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.774055,2.521211){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.806008,2.400568){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.836971,2.263348){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.867005,2.104257){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.367296,3.367296){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.414910,3.317301){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.460360,3.264674){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.503833,3.209123){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.545496,3.150303){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.585491,3.087807){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.623948,3.021143){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.660981,2.949715){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.696692,2.872790){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.731170,2.789451){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.764500,2.698529){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.796755,2.598507){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.828001,2.487357){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.858301,2.362289){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.887710,2.219313){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.401197,3.401197){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.447260,3.352910){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.491295,3.302171){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.533472,3.248720){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.573941,3.192250){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.612837,3.132400){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.650276,3.068737){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.686364,3.000745){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.721194,2.927790){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.754853,2.849091){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.787415,2.763666){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.818950,2.670255){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.849521,2.567211){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.879185,2.452317){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.907995,2.322487){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.935997,2.173250){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.433987,3.433987){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.478597,3.387294){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.521301,3.338313){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.562257,3.286810){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.601600,3.232508){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.639455,3.175088){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.675928,3.114169){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.711118,3.049297){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.745111,2.979923){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.777987,2.905374){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.809816,2.824817){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.840663,2.737198){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.870588,2.641158){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.899642,2.534904){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.927876,2.416004){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.955335,2.281034){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.628515,3.271208){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.665382,3.216029){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.700938,3.157627){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.735274,3.095600){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.768469,3.029471){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.800598,2.958657){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.831727,2.882444){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.861915,2.799939){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.891219,2.710011){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.919689,2.611189){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.947371,2.501519){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.974307,2.378323){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.000536,2.237789){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.758860,3.139854){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.791294,3.076680){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.822709,3.009244){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.853167,2.936930){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.882725,2.858976){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.911434,2.774427){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.939342,2.682064){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.966492,2.580293){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.992924,2.466980){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.018676,2.339166){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.844342,3.057395){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.874158,2.988600){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.903110,2.914720){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.931248,2.834943){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.958616,2.748246){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.985255,2.653313){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.011202,2.548413){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.036493,2.431205){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.061161,2.298413){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.923089,2.967521){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.950677,2.892006){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.977526,2.810319){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.003672,2.721362){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.029152,2.623711){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.053998,2.515483){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.078243,2.394103){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(3.996084,2.868764){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.021756,2.785074){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.046785,2.693735){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.071202,2.593207){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.095038,2.481431){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.118319,2.355572){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.039519,2.844968){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.064112,2.759174){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.088115,2.665322){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.111556,2.561742){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.134460,2.446179){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.081145,2.820593){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.104747,2.732586){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.127806,2.636079){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.150344,2.529255){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.172386,2.409639){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.143795,2.705271){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.165980,2.605955){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.187684,2.495677){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.181376,2.677189){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.202751,2.574895){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.223679,2.460932){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.217595,2.648296){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.238218,2.542840){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.252548,2.618543){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.272470,2.509722){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.286321,2.587878){};
\node[fill=black,shape=circle,inner sep=0.1pt] at(4.318990,2.556242){};
%\node at (4,6) {$\mathcal L_{\mathbb R}(\mathcal O_K (1000)) \cap \mathcal C_K (\varepsilon )$};
\node at (4,6) {$\mathcal L_{\mathbb R}(\mathcal O_K (L')) \cap \mathcal C_K (\ee)$};

